Learning to Manipulate Anywhere: A Visual Generalizable Framework For Reinforcement Learning

Can we endow visuomotor robots with generalization capabilities to operate in diverse open-world scenarios? In this paper, we propose \textbf{Maniwhere}, a generalizable framework tailored for visual reinforcement learning, enabling the trained robot policies to generalize across a combination of multiple visual disturbance types. Specifically, we introduce a multi-view representation learning approach fused with Spatial Transformer Network (STN) module to capture shared semantic information and correspondences among different viewpoints. In addition, we employ a curriculum-based randomization and augmentation approach to stabilize the RL training process and strengthen the visual generalization ability. To exhibit the effectiveness of Maniwhere, we meticulously design 8 tasks encompassing articulate objects, bi-manual, and dexterous hand manipulation tasks, demonstrating Maniwhere's strong visual generalization and sim2real transfer abilities across 3 hardware platforms. Our experiments show that Maniwhere significantly outperforms existing state-of-the-art methods. Videos are provided at https://gemcollector.github.io/maniwhere/.

==> figures/agg_results.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/cam_score.pdf}
  \caption{\textbf{Aggregated generalization score of autonomous driving.} We present the aggregated return of each method. SRM exhibits better performance to adapt to scenarios where image frequency varies dramatically.}
  \label{fig:sim-agg-results}
\end{figure}


==> figures/correlation.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=0.6\linewidth]{figures/corr.pdf}
  \caption{\textbf{Correlation between sim and real results.} Correlation coefficients Spearman and Pearson are shown in the bottom right. }
  \label{fig:corr}
\end{figure}


==> figures/cross-embodiment.tex <==
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=1.0\linewidth]{figures/cross-figure.pdf}
%   \caption{\textbf{Aggregated generalization score of autonomous driving.} We present the aggregated return of each method. SRM exhibits better performance to adapt to scenarios where image frequency varies dramatically.}
%   \label{fig:instances}
% \end{figure}


\begin{figure}[h]
    \centering
    \begin{minipage}[b]{0.7\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/cross-figure-new.pdf}
        \caption{\textbf{Feature Correspondence.} \ourshort can find the feature correspondence between different embodiments.}
        \label{fig:cross-figure}
    \end{minipage}
    \hfill 
    \begin{minipage}[b]{0.28\linewidth}
        \centering
        \scriptsize 
        \begin{tabular}{cc}
            \toprule
            Task & Success Rate \\
            \midrule
            LiftCube~(ur5) & $82$\scriptsize{$\pm 7$} \% \\
            LiftCube~(franka) & $59$\scriptsize{$\pm 28$}  \% \\
            \hline
        \end{tabular}
        \captionof{table}{\textbf{The experiment results of Cross Embodiment. }}
        \label{tab:cross-table}
    \end{minipage}
\end{figure}


==> figures/real-world.tex <==


\begin{figure}[h]
    \centering
    \begin{minipage}[t]{0.4\linewidth}
        \centering
        \vspace{0pt} 
        \includegraphics[width=\linewidth]{figures/real-world-bar.pdf}
        \caption{\textbf{Real-world Experiments.} Maniwhere can find the feature correspondence between different embodiments.}
        \label{fig:real-world}
    \end{minipage}
    \hfill 
    \begin{minipage}[t]{0.5\linewidth}
        \centering
        \vspace{8pt} 
        \begin{tabular}{lp{0.26\textwidth}}
            \toprule
            Ablation & Success Rate (\%) \\
            \midrule
            \cellcolor{cyan!20}Maniwhere & \cellcolor{cyan!20}85$\pm$7 \% \\
            w/o. multi-view objective & 28.8$\pm$8.3 \% \\
            w/o. STN & 78.6$\pm$4.2 \% \\
            w/ TCN   & 78.6$\pm$4.2 \% \\        
            \bottomrule
        \end{tabular}
        \caption{Experimental results showcasing various ablations.}
        \label{table:ablation}
    \end{minipage}
\vspace{-15pt}
\end{figure}

==> figures/robosuite.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/robosuite.pdf}
  \caption{The visualization of $3$ Robosuite tasks at diffrent viewpoints.}
  \label{fig:robo}
  \vspace{-10pt}
\end{figure}


==> figures/training-curve.tex <==
\begin{figure}[h]
  \centering
  \vspace{-10pt}
  \includegraphics[width=1.0\linewidth]{figures/train-curve.pdf}
  \caption{The training curves of \ourshort across tasks.}
  \label{fig:train-curve}
\end{figure}

